Efficient Approximation of Fractional Hypertree Width

We give two new approximation algorithms to compute the fractional hypertree width of an input hypergraph. The first algorithm takes as input $n$-vertex $m$-edge hypergraph $H$ of fractional hypertree width at most $\omega$, runs in polynomial time and produces a tree decomposition of $H$ of fractional hypertree width $O(\omega \log n \log \omega)$. As an immediate corollary this yields polynomial time $O(\log^2 n \log \omega)$-approximation algorithms for (generalized) hypertree width as well. To the best of our knowledge our algorithm is the first non-trivial polynomial-time approximation algorithm for fractional hypertree width and (generalized) hypertree width, as opposed to algorithms that run in polynomial time only when $\omega$ is considered a constant. For hypergraphs with the bounded intersection property we get better bounds, comparable with that recent algorithm of Lanzinger and Razgon [STACS 2024]. The second algorithm runs in time $n^{\omega}m^{O(1)}$ and produces a tree decomposition of $H$ of fractional hypertree width $O(\omega \log^2 \omega)$. This significantly improves over the $(n+m)^{O(\omega^3)}$ time algorithm of Marx [ACM TALG 2010], which produces a tree decomposition of fractional hypertree width $O(\omega^3)$, both in terms of running time and the approximation ratio. Our main technical contribution, and the key insight behind both algorithms, is a variant of the classic Menger's Theorem for clique separators in graphs: For every graph $G$, vertex sets $A$ and $B$, family ${\cal F}$ of cliques in $G$, and positive rational $f$, either there exists a sub-family of $O(f \cdot \log^2 n)$ cliques in ${\cal F}$ whose union separates $A$ from $B$, or there exist $f \cdot \log |{\cal F}|$ paths from $A$ to $B$ such that no clique in ${\cal F}$ intersects more than $\log |{\cal F}|$ paths.

==> menger.tex <==
\subsection{Clique Menger's Theorem} \label{sec-Mengers}
\begin{lemma}\label{lem:mainMengerSimplified}
Let $G$ be a graph on $n$ vertices, $A$ and $B$ be vertex sets in $G$, ${\cal F}$ be a set of cliques in $G$, and $f$ be a positive real. 
%\
Then, either there exists an $(A,B)$-separator $X$ such that $\rho_{G,\cal F}^*(X) \leq 8+4f\ln n$ or there exists a collection $P_1, P_2, \ldots, P_{\lceil f \cdot \log(|{\cal F}|) \rceil}$ of $A$-$B$ paths such that no clique in ${\cal F}$ intersects at least $6\log(|{\cal F}|)$ of the paths. \todo{modify bounds}
\end{lemma}
\todo{call LP2}
Let $\mathcal{P}$ be the set of $A$-$B$ paths in $G$. We now define an LP relaxation for the problem of finding an $A$-$B$ separator with minimum clique cover and also define its dual path packing LP.
\begin{equation*}
\tag{LP1}
\begin{array}{ll@{}ll}
\text{minimize}  & \displaystyle\sum\limits_{e\in \mathcal{F}} y_{e} &\\
\text{subject to}& \displaystyle\sum\limits_{e:e\cap V(P) \neq \emptyset}   &y_{e} \geq 1,  &\forall P\in \mathcal{P}\\
                 &                                                &y_{e} \in [0,1], &\forall e\in\mathcal{F}
\end{array}
\end{equation*}
\begin{equation*}
\tag{Dual}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum\limits_{P\in \mathcal{F}} z_{P} &\\
\text{subject to}& \displaystyle\sum\limits_{P:e\cap V(P) \neq \emptyset}   &z_{P} \leq 1,  &\forall e\in \mathcal{F}\\
                 &                                                &z_{P} \in [0,1], &\forall P\in\mathcal{P}
\end{array}
\end{equation*}
Let $\textsf{opt}$ be the optimum cost of LP1 and its dual.
\begin{lemma}
    If $\textsf{opt}\leq f$, then there is an $(A,B)$-separator $S$ of $G$ such that $\rho^*_{G,\mathcal{F}}(S)\leq 8+4f\ln n$.
\end{lemma}
\begin{proof}
    
Let $H$ be a hypergraph constructed from $G$ as follows: $V(H)=V(G)$, $E(H)=\mathcal{F}\cup E(G)$. Observe that $\gf{H}=G$. So each path in $G$ is a path in $\gf{H}$ and vice versa. Further any $S\subseteq V(H)$ is an $(A,B)$-seperator of $H$ if and only if $S$ is an $(A,B)$-separator of $G$ and $\rho^*_{H,\mathcal{F}}=\rho^*_{G,\mathcal{F}}(S)$. So to prove the Lemma, we find an $(A,B)$-separator for $H$ with $\rho^*_{H,\mathcal{F}}\leq 8+4fln n$.

If $\hy$ is a feasible solution to \text{LP1} of cost at most $f$, we now show that $x:V(H_G)\rightarrow [0,1]$, $x(v)=\sum_{e:e\cap v\neq \emptyset}\hy_e$ is a fractional $(A,B)$-separator in $H$ such that $\rho^*_{H,\mathcal{F}}(x)\leq f$.
%
Since $\hy$ is a feasible solution to $LP1$ of cost at most $f$, for each $A$-$B$ path $P$ in $G$, $\sum_{e:e\cap V(P)\neq \emptyset}\hy_e\geq 1$.
%
Let $P\in \mathcal{P}$ be an $A$-$B$ path. Observe that $\sum_{v\in P}x(v)=\sum_{v\in P}\sum_{e:e\cap v\neq \emptyset}\hy_e\geq \sum_{e:e\cap V(P)\neq \emptyset}\hy_e\geq 1$. Thus $dis_{H,x}(A,B)\geq 1$. Further observe that by definition of $x$, $\hy$ is a fractional $\mathcal{F}$-edge cover of $x$. Therefore $x$ is a fractional $(A,B)$-separator with $\rho^*_{H,\mathcal{F}}(x)= \sum_{e\in E(H)}\hy_e\leq f$. 

By Theorem~\ref{theorem:ab-sep-stronger}, there exists an $(A,B)$-separator $S$ of $H$ satisfying $\rho_{H,\mathcal{F}}^*(S) \leq \min\{8 + 4 \ln \alpha_H(R), 6 \mu_H\} \cdot \rho_{H,\mathcal{F}}^*(x)\leq 8+4\ln n\cdot \rho_{H,\mathcal{F}}^*(x)\leq 8+4f\ln n $. This complete the proof.

% \begin{theorem}\label{theorem:ab-sep-stronger}
% Given a hypergraph $H$, two sets $A,B \subseteq V(H)$, a fractional $(A,B)$-separator $x: V(H) \rightarrow [0,1]$ with $\mathsf{supp}(x) = R$, and a set $E \subseteq E(H)$, one can compute in $\lVert H \rVert^{O(1)}$ time an $(A,B)$-separator $S \subseteq R$ satisfying that $\rho_{H,E}^*(S) \leq \min\{8 + 4 \ln \alpha_H(R), 6 \mu_H\} \cdot \rho_{H,E}^*(x)$.
% \end{theorem}
\end{proof}

\begin{lemma}
    If $\textsf{opt}>f$, then there exists a collection $P_1, P_2, \ldots, P_{\lceil f \cdot \log(|{\cal F}|) \rceil}$ of $A$-$B$ paths in $G$ such that no clique in ${\cal F}$ intersects at least $6\log(|{\cal F}|)$ of the paths. 
\end{lemma}
\begin{proof}
  Let $\hz$ be an optimum solution to the dual LP of cost $\sum_{P\in \cP}\hz_P = \textsf{opt}>f$. For each path $P\in \cP$, we define the function $z':\cP\rightarrow [0,1]$ as $z'(P):=\frac{\hz_P}{\sum_{Q\in \cP}\hz_Q}$ for each $P\in \cP$. Observe that $\sum_{P\in \cP}z'(P)=1$ and thus $z'$ is a probability distribution on $\cP$. Let $t=\log{|\cF|}$, we sample independently one by one $t\cdot f$ paths $P_1, P_2, \ldots, P_{\lceil tf \rceil}$  from the distribution $z'$. 
%
  For each $e\in \mathcal{F}$ and $i\in \ell$, the following holds $$Pr[P_i\cap e\neq\emptyset]= \sum_{P:e\cap V(P)\neq \emptyset}z'(P)=\sum_{P:e\cap V(P)\neq \emptyset}\frac{z_P}{\sum_{Q\in \cP}\hz_Q}\leq \frac{1}{\sum_{Q\in \cP}\hz_Q}\cdot\sum_{P:e\cap V(P)\neq \emptyset}z_P\leq \frac{1}{f}$$.

Let $X_{e,i}$ be an indicator random variable that denotes whether $P_i$ intersects $e\in \cF$ or not. Further let $X_e=\sum_{i\in[\ell]}X_{e,i}$  denote the number of paths in $\{P_1,\cdots,P_\ell\}$ that intersect $e$. 
$$E[X_e]=\sum_{i\in\ell}E[X_{e,i}]\leq \sum_{i\in\ell} 1\cdot \frac{1}{f} \leq \ell.\frac{1}{f}\leq \frac{t.f}{f}\leq t$$

We use the following variant of Chernoff bounds, $Pr[X_e\geq R]\leq 2^{-R}, R\geq 2e\mu$ since $X_e$ is the sum of independent random variables. 
%
We have $t=\log{|\cF|}$,
$$Pr[X_e\geq 6t]= Pr[X_e\geq 6 \log{|\cF|}]\leq 2^{-6\log{|\cF|}}\leq \frac{1}{|\cF|^{6}}$$
% By Chernoff bounds, PrX ≥ R ≤ 2−R for R ≥ 2eμ (≈ 5.44μ)
\end{proof}



    % Let $d_{AB}=\min_{a\in A, b\in B} dis_{H,x}(a,b)$ and let $P=\{v_1,\cdots,v_\ell\}$ be a path between $a\in A$, $b\in B$ having $dis_{H,x}(a,b)=d_{AB}$. Observe that $P$ is an induced path in $H$, that is there is no edge between two vertices $v_i,v_{j}\in P$ having $j\geq i+2$. If not, there exists a path $P'$ between $a$ and $b$ having $\sum_{v\in P'}x(v)<dis_{H,x}(a,b)$, which cannot happen. Thus every $e\in E(H_G)$ intersects at most two vertices in $P$, that is $|e\cap V(P)|\leq 2$. Thus we have 
% \begin{equation*}
% \begin{array}{ll@{}ll}
% \text{minimize}  & \displaystyle\sum\limits_{j=1}^{m} w_{j}&x_{j} &\\
% \text{subject to}& \displaystyle\sum\limits_{j:e_{i} \in S_{j}}   &x_{j} \geq 1,  &i=1 ,\dots, n\\
%                  &                                                &x_{j} \in \{0,1\}, &j=1 ,\dots, m
% \end{array}
% \end{equation*}

